MCTS-EP: Empowering Embodied Planning with Online Preference Optimization

This paper introduces MCTS-EP, an online learning framework that combines large language models (LLM) with Monte Carlo Tree Search (MCTS) for training embodied agents. MCTS-EP integrates three key components: MCTS-guided exploration for preference data collection, efficient multi-modal reasoning mechanism, and iterative training pipeline based on preference optimization. We theoretically prove that MCTS-EP achieves better performance bounds than conventional on-policy algorithms when the loss function is strongly convex, and demonstrate that it can be formulated as a search-enhanced variant of GAIL. MCTS-EP achieves state-of-the-art performace across serval benchmarks. In ALFWorld, it achieves 92% and 87% success rates for textual and visual tasks. In WebShop, it reaches an average reward of 0.81. MTCS-EP also reduces average interaction steps from from 18.7/19.5 to 10.2/9.9 steps in visual ALFWorld.Code available at: https://github.com/xuhang-2/Embodied-Agent-Planning

==> sec/0_abs.tex <==
\begin{abstract}
xxx
\end{abstract}

==> sec/1_intro.tex <==
\setlength{\parindent}{2em}

\section{Introduction}
Recently, large language models (LLMs) trained on internet-scale data have demonstrated strong capabilities in commonsense reasoning\cite{touvron2023llama, bai2023qwen, team2024gemma, wei2022chain}. Furthermore, vision-language models (VLMs) can effectively bridge the gap between language instructions and visual observations, enabling more robust multi-modal reasoning \cite{wang2024qwen2, li2023blip, liu2024visual, zhu2023minigpt}. Building on these advancements, embodied agents can now perform complex decision-making tasks in interactive environments based on general commonsense knowledge \cite{wu2023tidybot, li2024llava, stella2023can}. 

A key challenge is that agents must reason over multi-modal information and sequentially decompose tasks into actionable steps to efficiently interact with their environment \cite{jansen2020visually, huang2022language, li2022pre}. Recent works have explored using techniques like Monte Carlo Tree Search (MCTS) \cite{coulom2006efficient, kocsis2006bandit} to enhance LLM reasoning by enabling strategic exploration and decision-making in sequential tasks \cite{zelikman2024quiet, zhao2024large, zhang2024rest}. But these methods are not exclusively focused on embodied scenarios.

Some recent works have focused on improving embodied agents through feedback, preference optimization, and cross-modal learning. Reflexion \cite{shinn2024reflexion} proposes using linguistic feedback and episodic memory to enable agents to learn from trial-and-error without expensive model fine-tuning. IPR \cite{xiong2024watch} introduces step-level rewards and preference optimization to provide detailed supervision instead of outcome-based signals. SayCan \cite{ahn2022can} uses visual navigation to collect information in the house to generate grounded plans. EMMA \cite{yang2024embodied} takes a cross-modality approach by distilling LLM's knowledge from text world to guide visual world learning. 

Despite advances in embodied planning algorithms, several limitations remain.
First, generating high-quality data is a persistent challenge. Most methods rely on imitation learning \cite{hussein2017imitation}, which depends entirely on expert demonstrations. These approaches lack sufficient exploration of interactive environments and fail to leverage insights from trial-and-error failures \cite{song2024trial}. While IPR \cite{xiong2024watch} introduces a method for collecting preference pairs, it relies on random sampling without integrating LLMs' knowledge or their ability to actively explore.
Second, many existing works focus on TextWorld \cite{cote2019textworld}, where agents depend on structured textual feedback and predefined candidate actions to guide planning. However, real-world scenarios require robots to independently analyze the environment through visual input from cameras to infer both candidate actions and environmental feedback. EMMA \cite{yang2024embodied} partially addresses this limitation through a multi-modal approach but struggles with repeated trial-and-error attempts, which are impractical in real-world applications where mistakes can be costly.
Lastly, methods like IPR leverage direct preference optimization (DPO) \cite{rafailov2024direct} for preference learning. Existing approaches often rely on static datasets or random sampling to collect preference pairs, limiting the model to passively learn from predefined trajectories without actively interacting with the environment \cite{xiong2024watch}. This results in offline models that cannot adapt or improve beyond the constraints of the original data. In contrast, an online framework allows the model to iteratively generate and incorporate preference data through its own exploration, enabling continuous refinement of planning capabilities and better generalization to unseen scenarios.


To address these limitations, we propose a multi-modal framework (MCTS-DPO) that generates preference data and trains LLMs for embodied agents online.  
MCTS-DPO includes three components: 
1) Preference Data Collection based on MCTS: We use MCTS and Supervised Fine Tuned (SFT) LLM/VLM as base model, generating preference action pair. Besides, we make a series of improvements to MCTS to improve the efficiency of data collection, 
2) Selective State Representation for Multi-Modal Reasoning: We propose a new multi-modal planing pipeline that balances reasoning speed with memory utilization. 
3) MCTS-Enhanced DPO: We design an MCTS-Enhanced DPO framework that combines expert fine-tuning, preference data collection, and iterative optimization to improve model accuracy and task efficiency.


The main contributions of this work can be summarized as:
\begin{enumerate}
    \item Preference Data Collection based on MCTS: We propose an improved efficient data collection method from MCTS, enabling faster and more effective preference data generation.
    \item MCTS-Enhanced DPO: We design a pipeline that maintains inference efficiency while incorporating memory during reasoning. The training process approximates offline DPO as single- or multi-round online training, improving model performance in both accuracy and task efficiency.
    \item We evaluate MCTS-DPO and compare it with text-based and vision-based methods on the ALFWorld benchmark \cite{shridhar2020alfworld}. Experimental results show that our method consistently achieves the highest task success rate and the shortest task completion steps across both textual and visual settings, outperforming state-of-the-art (SOTA) methods. Notably, our approach completes tasks in a single attempt without relying on trial-and-error.
\end{enumerate}



==> sec/2_relatedWork.tex <==
\section{Related Work}
\textbf{Long-horizon Reasoning with Language Models.}
Recent large language models have significantly advanced long-horizon reasoning  \cite{touvron2023llama, bai2023qwen}. Chain-of-thought prompting \cite{wei2022chain} enables step-by-step task decomposition. Several works combine MCTS with LLM for systematic exploration \cite{zelikman2024quiet, zhao2024large, zhang2024rest}. Reflexion \cite{shinn2024reflexion} uses feedback and memory for iterative improvement. However, these methods primarily target language-only tasks. Vision language models \cite{wang2024qwen2, li2023blip} bridge visual and linguistic understanding, enabling multi-modal reasoning \cite{chen2024spatialvlm,chen2024large}.


\noindent \textbf{Task Planning for Embodied Agents.}
Task planning for embodied agents requires decomposing high-level goals into executable action sequences while considering environmental constraints. Traditional approaches rely heavily on structured action spaces and expert demonstrations \cite{hussein2017imitation}, limiting their applicability in dynamic environments. Recent works like SayCan \cite{ahn2022can} have made progress incorporating visual grounding for more robust planning, while IPR \cite{xiong2024watch} introduces preference optimization to provide fine-grained supervision. EMMA \cite{yang2024embodied} takes a cross-modal approach to transfer knowledge from text to visual domains, though it often requires multiple attempts to complete tasks successfully.



==> sec/3_method.tex <==
\section{Method}
\begin{figure}[ht] % 创建浮动环境
    \centering % 图片居中
    \includegraphics[width=1\textwidth]{framework.png} % 插入图片，设置宽度为页面宽度的50%
    \caption{Framework of MCTS-DPO} % 添加图片标题
    \label{fig:example} % 添加标签，便于引用
\end{figure}

\subsection{Preliminary}
In this section, we introduce the basic settings of MCTS-DPO. It can be formulated as a partially observable Markov decision process (POMDP), defined by a tuple $\langle \mathcal{U}, \mathcal{A}, \mathcal{O}, \mathcal{S}, \mathcal{T}, \mathcal{R} \rangle$. $\mathcal{U}$ is instruction space, $u_t \in \mathcal{U}$ is a natural language instruction, an example is "put a clean pan in countertop". $\mathcal{A}$ is action space, $a_t \in \mathcal{A}$ is action in step t. $\mathcal{O}$ is observation space. $o_t \in \mathcal{O}$ is observation in step t, which can be verbal or vision. $\mathcal{S}$ is state space. $s_t \in \mathcal{S}$ can be written as:
\begin{equation}
s_t=(u, a_1, o_1, ..., a_t, o_t),
\end{equation}
$T: S \times A \times S \rightarrow [0,1]$ is the transition function. $R: S  \rightarrow [0,1]$ is the reward function. In this paper, we use outcome reward function, only applying to terminal state. Besides, we define initial policy model ${\pi}_{\theta_0}$ and policy model ${\pi}_{\theta_i}$ as LLMs or VLMs. The objective function for
\begin{equation}
\min_{\theta_i} \mathbb{E}_{s_t \sim \mathcal{S}} [D_{KL}(\pi_{\theta_i}(a^{\ast}_t|s_t) \| \pi^*(a^{\ast}_t|s_t))],
\end{equation}
where $\pi_{\theta_i}(a^{\ast}_t|s_t)$ is the predicted action distribution, $\pi^{\ast}(a^{\ast}_t|s_t)$ is the optimal policy distribution, $a^{\ast}_t$ is the ground truth action.

\subsection{Preference Data Collection based on MCTS}
\label{subsec:data_generation}
To generate action-level preference data, we decompose the planning process into several phases in the React-style \cite{yao2022react}. In every planning process, we sample candidate action from probability distribution of ${\pi}_{\theta_i}$.  We employ MCTS to collect preference data, where MCTS acts as an implicit reward model. This approach offers several advantages: (1) it provides dynamic evaluation through look-ahead search rather than static scoring, (2) it naturally captures long-term consequences of actions through value propagation, and (3) it requires no additional training of separate reward models. After constructing the Monte Carlo search tree, we extract preference data from each branching node. Specifically, at each decision point $s_t$, we obtain preference pairs $(a_i, a_j)$ where actions are scored by their action value estimate $Q(s_t,a)$. 

The MCTS algorithm starts from a root node $s_0$ representing the initial state, and iteratively builds a search tree through repeated search episodes. Each episode consists of four consecutive phases: selection (selecting promising nodes using Predictor + Upper Confidence bounds applied to Trees (PUCT) \cite{rosin2011multi}), expansion (adding new nodes to the tree), simulation (evaluating new states through rollouts), and backup (propagating values back through the tree). Below, we detail each phase.

\textbf{Selection}: Starting from the root node, the algorithm recursively selects child nodes until reaching a leaf node, using PUCT to balance exploration and exploitation : 
\begin{equation}
    s_t^{\ast} = argmax_{s_t \in \mathcal{S}} \left[Q(s_t,a) + c_{puct}\pi_{{\theta}_{i}}(a|s_t)\sqrt{\frac{N(s_t)}{1 + N(s_t,a)}}\right],
\end{equation}
where $Q(s_t,a)$ is the estimated action value, 
$N(s_t)$ denotes the visit count of state $s_t$,
$N(s_t,a)$ is the visit count of action $a$ at state $s_t$, 
$c_{puct}$ is the exploration coefficient, 
$\pi_{\theta}(a|s_t)$ is the prior probability of action $a$ given by the policy model.

\textbf{Expansion}: Unlike standard MCTS expansion, we introduce a self-critic \cite{zhang2024rest} to improve expansion efficiency. For each leaf node $s_t$ reached during selection, we first employ the critic LLMs to evaluate whether expansion is necessary:
\begin{equation}
\text{expand}(s_t) = \begin{cases}
\text{true} & \text{if } \pi_{{\theta}_{c}}(s_t) > \tau \\
\text{false} & \text{otherwise}, 
\end{cases}
\end{equation}
\noindent where critic LLMs $\pi_{{\theta}_{c}}$ assesses the node's potential value based on current state and context, and $\tau$ is a threshold parameter. If $\text{expand}(s_t)$ returns true, the algorithm proceeds with standard expansion by sampling c actions from the policy model $\pi_{\theta}(a|s_t)$ and adding corresponding child nodes to the tree. The tree expansion is performed by sampling $c$ actions according to the policy network $\pi_{\theta}$, where $c$ represents the computational budget that determines the branching factor. Specifically, we select actions through:
\begin{equation}
a_{t+1}^{(1)}, ..., a_{t+1}^{(c)} = argmax_{A} \pi_{\theta}(A | s_t^{\ast}),
\end{equation}
where $s_t^{\ast}$ denotes the leaf node selected for expansion, and each sampled action $a_{t+1}^{(i)}$ leads to the creation of a new child node in the search tree.
Otherwise, the node is marked as non-expandable and excluded from future selection paths until conditions change.

\textbf{Simulation}: After expanding a node, we enhance the traditional rollout process by leveraging LLM's generative capabilities. Instead of using simple random policies or pre-defined heuristics, we employ the greedy algorithm to perform guided trajectory sampling:
\begin{equation}
s_{t+1}^{(i)} = (s_t^{\ast}, a_{t+1}^{(i)}, o_{t+1}^{(i)}), \quad  i = 1, \dots, c ,
\end{equation}
\begin{equation}
a_{t+2}^{(i)}  = argmax_A \pi_{\theta_{i}}(A|s_{t+1}^{(i)}) ,
\end{equation}
where $\gamma$ is the discount factor. This approach combines the strategic reasoning of LLMs with the exploratory nature of MCTS rollouts, potentially leading to more informative value estimates. The simulation continues until either reaching a terminal state or the maximum depth $d_{max}$, at which point the reward function $r_o$ evaluates the final state to provide reward:
\begin{equation}
r_o(s_{\text{terminal}}) = \begin{cases}
1 & \text{if task completed} \\
0.5 & \text{if task partially completed} \\
0 & \text{if task not completed}.
\end{cases}
\end{equation}

Additionally, we maintain a success trajectory buffer $\mathcal{B} = \{(u, a_1, ..., o_T)^i\}_{i=1}^N$ that stores all successful solution paths discovered in the Monte Carlo search tree, where $N$ is the number of successful trajectories. These high-quality trajectories serve as valuable training data for subsequent model improvement and can be used to fine-tune both the policy network $\pi_{\theta_{i}}$.

\textbf{Backup}: After each simulation, the reward are propagated back through the selected path to update node statistics. For each node $s_t$ in the backup path, we update its statistics as follows:
\begin{equation}
N(s_t) \leftarrow N(s_t) + 1 ,
\end{equation}
\begin{equation}
V(s_t) \leftarrow V(s_t) + \gamma \cdot r(s_{t+1}) ,
\end{equation}
\begin{equation}
Q(s_t, a_t) \leftarrow Q(s_t, a_t) + \frac{1}{N(s_t, a_t)}[V(s_{t+1}) - Q(s_t, a_t)] ,
\end{equation}
where $N(s_t)$ is the visit count for state $s_t$,  $Q(s_t, a_t)$ is the action value estimate, $V(s_{t+1})$ is the simulated value from the child node, $r(s_{t+1})$ is discount reward propagated back through the simulation path with discount factor $\gamma$.

We obtain two valuable datasets from the constructed search tree:
\begin{enumerate}
    \item Preference Pairs Dataset $\mathcal{P}$: At each branching point in the tree, actions are ranked according to their action value estimates $Q(s_t, a_t)$. By comparing these values, we construct preference pairs where higher-valued actions are labeled as preferred over lower-valued ones.
    \item Success Trajectory Dataset $\mathcal{B}$: We maintain a trajectory buffer $\mathcal{B}$ containing complete successful solution paths discovered during the search. Each trajectory in $\mathcal{B}$ represents a sequence of observation-action pairs $(s_0, a_0, ..., o_T)$.
    
\end{enumerate}

\subsection{Selective State Representation for Multi-Modal Reasoning}
In real-world scenarios, robot observations are primarily derived from continuous camera feeds, resulting in a stream of visual inputs. Specifically, at each timestep \(t\), the agent receives a raw image observation \(o_t\). The policy model \(\pi_{\theta_i}\) predicts action \(a_t\) and extracts textual description \(\tau_t\) from observation \(o_t\)

\begin{equation}
a_t, \tau_t = \pi_\theta(s_t),
\end{equation}
where $s_t$ is the history of prior actions and image observations, and \(\tau_t\) is the textual information extracted from \(o_t\) (e.g., object labels or spatial context).

For long-horizon tasks, storing all historical observations for reasoning is computationally expensive and requires excessive memory. Instead of storing the complete history of image observations \(\{o_1, o_2, \dots, o_{t-1}\}\), we retain only the textual descriptions \(\{\tau_1, \tau_2, \dots, \tau_{t-1}\}\) and associated actions. At timestep \(t\), the current image \(o_t\) is used directly by the policy \(\pi_\theta\) to predict the next action \(a_t\) and extract \(\tau_t\), which is then appended to the state for future reasoning.

Thus, the state update at each timestep can be expressed as:
\begin{equation}
s_{t-1} = (u,a_1, \tau_1,..., a_{t-1}, \tau_{t-1}), 
\end{equation}
\begin{equation}
s_t = s_{t-1} \cup \{a_t, o_t\}.
\end{equation}

The memory-efficient pipeline selectively retains textual observations while discarding raw images, allowing VLMs to preserve essential information and complete long-horizon tasks in a single attempt without relying on trial-and-error approaches.

\subsection{MCTS-Enhanced DPO}
MCTS-DPO is designed to iteratively improve agent's performance by MCTS for exploration and data generation. Staring from an initial policy model $\pi_{\theta_0}$, the framework alternates between data generation and model updates. At iteration \(t\), MCTS-DPO performs following steps:

\begin{enumerate}
    \item Data generation with MCTS (Section~\ref{subsec:data_generation}): Using current policy model $\pi_{\theta_{i}}$, MCTS is applied to explore environment and generate success trajectory data $\mathcal{B}$ and preference pairs data $\mathcal{P}$.
    \item Imitation learning using expert trajectories: The training process begins by leveraging expert trajectories $\mathcal{D}_\text{expert}$ for pre-trained LLMs/VLMs to initialize policy model $\pi_{\theta_{0}}$.
    \item Fine-tuning with success trajectory data $\mathcal{B}$: Success trajectory data is used to fine-tune the policy model \(\pi_{\theta_i}\), incorporating successful attempt to enhance model performance through iterative updates.
    \item Direct preference optimization with preference data $\mathcal{P}$: The preference pairs data \(\mathcal{P}_t\) is used to further fine-tune the model, aligning the policy with task-specific preferences. 
\end{enumerate}


\subsubsection{Imitation Learning with Expert Trajectory}
The first stage of the process involves Supervised Fine-Tuning (SFT) using a given dataset of expert demonstrations $\mathcal{D}_\text{expert}$. In embodied scenarios, gathering large quantities of high-quality demonstrations is often costly and challenging, especially for tasks that require human expertise or physical interactions with the real world. As a result, the primary utility of small datasets in this context lies in training initial policy model $\pi_{\theta_{0}}$ to produce outputs in the correct format and adhere to task-specific conventions. The performance of policy model $\pi_{\theta_{0}}$ relies on a continuous improvement process.

Specifically, we denote expert trajectory $e_u \in \mathcal{D}_\text{expert}$ as $e_u = (u, a_1^{\ast}, a_2^{\ast},... , a_k^{\ast})$, where $a_t^{\ast}$ is the best action at step t. Based on $e_u$, we can get expert terminal state $s_{u_t} = (u, a_1^{\ast}, o_1, ..., a_k^{\ast}, o_k)$. Our object is to minimize loss function:
\begin{align}
\mathcal{L}_{\text{SFT}}(\theta) &= -\mathbb{E}_{e_u \sim \mathcal{D}_\text{expert}} [\log \pi_{\theta}(e_u|u)] \nonumber \\
&= -\mathbb{E}_{e_u \sim \mathcal{D}_\text{expert}} \left[\sum_k \log \pi_{\theta}(a_k|s_{u_{k-1}})\right],
\end{align}
where $s_{u_{k-1}} = (u, a_1^{\ast}, o_1, ..., a_{k-1}^{\ast}, o_{k-1})$ represent current state at step $t-1$. This loss encourages the policy model $\pi_{\theta}$ to maximize the likelihood of expert actions $a_t^{\ast}$. 

Through the minimization of $\mathcal{L}_{\text{SFT}}(\theta)$, the model learns to generate actions in alignment with expert demonstrations, providing a robust starting point for further optimization and exploration. This process is particularly important in embodied scenarios, where data scarcity and task complexity demand efficient and effective learning from limited resources.

\subsubsection{Fine-Tuning with Success Trajectory Data}
After obtaining the initial policy model \(\pi_{\theta_0}\) through imitation learning on expert trajectory, MCTS leverages the initial policy \(\pi_{\theta_0}\) to guide the search process and generate trajectories that explore the state-action space. We can get preference pairs dataset $\mathcal{P}$ and success trajectory dataset $\mathcal{B}$. Each success trajectory in $\mathcal{B}$ can be seen as a terminal state \(s_T\) when the trajectory satisfies task-specific objectives. \(s_T\) is composed of a sequence of observation-action pairs. 

Formally, the objective is to minimize the negative log-likelihood:
\begin{equation}
\mathcal{L}_\text{SFT}(\theta) = -\mathbb{E}_{s_T \sim \mathcal{B}} \left[ \sum_{t=1}^T \log \pi_\theta(a_t | s_{t-1}) \right].
\end{equation}

This objective encourages the policy model \(\pi_\theta\) to assign higher probabilities to actions that lead to successful outcomes. For multi-modal environment, the history trajectory can be replaced with the representation method in Memory-Efficient Multi-Modal Reasoning, enabling the model to effectively integrate and reason across diverse modalities while maintaining computational efficiency.

Compared to the initial imitation learning stage, fine-tuning with success trajectories enables the policy to adapt based on its own exploration of the environment. The use of MCTS allows for the discovery of trajectories that may not be present in the expert dataset \(\mathcal{D}_\text{expert}\), enabling the policy to generalize beyond the constraints of the expert demonstrations. Besides, since the outcome reward model $r_o$ directly evaluates whether a trajectory achieves the task objective, the fine-tuning process optimizes the policy with respect to task-specific goals rather than purely imitating expert behavior.

\subsubsection{Direct Preference Optimization with Preference Data}
The last component is Direct Preference Optimization(DPO), improving the policy model's commonsense of world. DPO directly enhances the policy model’s efficiency in completing tasks, which can manifest as reducing the number of steps required to find a object.

To achieve this alignment, preference data \(\mathcal{P}\) is utilized. Each preference in \(\mathcal{P}\) is represented as a tuple \((a_t^w, a_t^l, s_{t-1})\), where \(a_t^w\) denotes the winning action that leads to a higher reward,  \(a_t^l\) denotes the losing action with a lower reward,  \(s_{t-1}\) represents the action-observation history.  

The preference data is used to construct a contrastive objective that encourages the policy to assign higher probabilities to \(a_t^w\) over \(a_t^l\) in the same context \(s_{t-1}\). Formally, the DPO objective is defined as:  
\begin{equation}
\mathcal{L}_\text{DPO}(\theta) = -\mathbb{E}_{(a_t^w, a_t^l, s_{t-1}) \sim \mathcal{P}} \left[
\log(\sigma(\beta \cdot (\log(\frac{\pi_\theta(a_t^w|s_{t-1})}{\pi_{ref}(a_t^w|s_{t-1})}) - \log(\frac{\pi_\theta(a_t^l|s_{t-1})}{\pi_{ref}(a_t^l|s_{t-1})}))))
\right], 
\end{equation}
where \(\pi_\theta(a_t^w | s_{t-1})\) and \(\pi_\theta(a_t^l | s_{t-1})\) are the probabilities assigned by the policy \(\pi_\theta\) to $a_t^w$ and $a_t^l$, respectively, conditioned on the state \(s_{t-1}\).

The preference data \(\mathcal{P}\) is typically derived from policy model exploration or expert demonstrations. For a given state \(s_{t-1}\), the model evaluates multiple candidate actions and their resulting outcomes. A preference is constructed whenever \(Q(s_t, a_t^w) > Q(s_t, a_t^l)\), indicating that \(a_t^w\) leads to a more favorable outcome compared to \(a_t^l\). The policy model uses these preferences to refine its policy during training, ensuring that future decisions reflect the learned task-specific priorities.

\begin{algorithm}
\caption{MCTS-Enhanced DPO}
\label{alg:mcts-dpo}

\begin{algorithmic}[1]
\Require Initial policy model $\pi_{\theta_0}$, expert demonstrations $\mathcal{D}_\text{expert}$
\Ensure Optimized policy model $\pi_{\theta}$

\State \textbf{Phase 1: Imitation Learning}
\For{$e_u=(u,a_1^*,...,a_k^*) \in \mathcal{D}_\text{expert}$}
    \State $s_{u_{k-1}} \gets (u,a_1^*,o_1,...,a_{k-1}^*,o_{k-1})$ 
    \State Minimize $\mathcal{L}_\text{SFT}(\theta) = -\sum_k \log \pi_{\theta}(a_k|s_{u_{k-1}})$
\EndFor

\State \textbf{Phase 2: Iterative Improvement}
\For{iteration $i=1$ to $T$}
    \State $\mathcal{B}, \mathcal{P} \gets \text{MCTS}(\pi_{\theta_i})$ \Comment{Step 1: Generate success and preference data}
    
    \For{$s_T \in \mathcal{B}$}
        \State Minimize $\mathcal{L}_\text{SFT}(\theta) = -\sum_{t=1}^T \log \pi_\theta(a_t|s_{t-1})$
        \Comment{Step 2: Fine-tune with Success Trajectories}
    \EndFor
    \For{$(a_t^w, a_t^l, s_{t-1}) \in \mathcal{P}$}
        \State $p_w \gets \log(\pi_\theta(a_t^w|s_{t-1})/\pi_\text{ref}(a_t^w|s_{t-1}))$
        \State $p_l \gets \log(\pi_\theta(a_t^l|s_{t-1})/\pi_\text{ref}(a_t^l|s_{t-1}))$
        \State Minimize $\mathcal{L}_\text{DPO}(\theta) = -\log(\sigma(\beta(p_w - p_l)))$ \Comment{Step 3: Direct Preference Optimization}
    \EndFor
    
    \State $\theta_{i+1} \gets \theta_i$ \Comment{Update model parameters}
\EndFor

\Return $\pi_{\theta}$
\end{algorithmic}
\end{algorithm}


Complete MCTS-Enhanced DPO algorithm is summarized in Algorithm \ref{alg:mcts-dpo}. The algorithm combines imitation learning, fine-tuning with success trajectories, and direct performance optimization to iteratively refine the policy model. MCTS-guided exploration enables the model to learn from successful experiences. DPO's preference-based optimization helps the model understand and incorporate task-specific preferences. This integrated approach addresses the challenges of both exploration and optimization in complex embodied environments.




==> sec/4_theory.tex <==
\section{Theory Analysis}
\subsection{MCTS Performance Bounds}
In this section, we provide theoretical performance guarantees for MCTS-based policies compared to conventional on-policy algorithms. Our analysis demonstrates that MCTS exhibits superior bounds under certain conditions.

\begin{theorem}
\label{theorem:Performance}
Let $\pi_{\theta}$ be a policy represented by a language model and $\pi_{mcts}$ be the policy derived from Monte Carlo Tree Search with Upper Confidence Bounds. For any state $s$, if the loss function $l$ is strongly convex, then:
$$\mathbb{E}[l(s, \pi_{mcts})] \leq \mathbb{E}[l(s, \pi_{\theta})].$$
\end{theorem}

The complete proof of Theorem \ref{theorem:Performance} is presented in Appendix \ref{app:Performance}. Our proof follows a similar structure to DAgger \cite{ross2011reduction}, but extends it to the MCTS setting. This theoretical guarantee provides a formal foundation for the empirical success of MCTS in various decision-making scenarios and offers insights into why MCTS-enhanced policies tend to outperform standard policy networks.





\subsection{MCTS-DPO as Search-Enhanced GAIL Variant}
Generative Adversarial Imitation Learning (GAIL) \cite{ho2016generative} optimizes policies via adversarial training to match the state-action occupancy measure of expert demonstrations. Traditional GAIL uses a discriminator to distinguish between expert and learned policy trajectories. In this section, we show MCTS-DPO can be viewed as a search-enhanced variant of GAIL, where the MCTS serves as an implicit discriminator through its value estimation process. This connection is formally established in the following theorem:

\begin{theorem}
\label{theorem:gail}
Let cost regularization is $$\psi(a) = c*\frac{\sqrt{ln t}}{t*\rho_{\pi}(s,a)} + \mathbb{E}_{\pi_E}[\log \pi_{E}(a|s)],$$ MCTS-DPO framework can be approximately formulated as $\text{RL} \circ \text{IRL}_{\psi}(\pi_E)$ in the GAIL framework: $$\text{RL} \circ \text{IRL}_{\psi}(\pi_E) = argmin_{\pi \in \Pi} \, -H(\pi) + \psi^*(\rho_{\pi} - \rho_{\pi_E}),$$ 
where $H(\pi) = \mathbb{E}_{\pi}[-\log \pi(a|s)]$, $\rho_{\pi}$ is occupancy measure of  policy $\pi$ and $\psi^*$ is convex conjugate function of $\psi$.
\end{theorem}

The complete proof can be found in Appendix \ref{app:gail}. This formulation reveals a two-stage optimization process. The Lower Confidence Bound LCB \cite{rashidinejad2021bridging} policy first generates a value function that serves as the cost function in IRL\cite{ng2000algorithms}. DPO maximizes the log-probability difference between preferred and rejected actions through entropy-regularized optimization.This theoretical analysis leads to the following important corollary:

\begin{corollary}
\label{corollary:two_stage}
The MCTS search process in MCTS-DPO implicitly performs cost function learning, while the DPO optimization corresponds to policy improvement with respect to this learned cost function. This two-stage process ensures both exploration through MCTS and effective policy updates through DPO.
\end{corollary}


==> sec/5_experiment.tex <==
\section{Experiments}
In this section, we conduct serval experiments to validate the effectiveness of MCTS-DPO. Our framework demonstrates better performance compared to baselines and SOTA methods. 
\subsection{Experiment Settings}

\textbf{Datasets} We evaluate MCTS-DPO on the ALFWorld \cite{shridhar2020alfworld} benchmark, which extends the ALFRED \cite{shridhar2020alfred} dataset. ALFWorld uses the AI2-THOR \cite{kolve2017ai2} simulator to create a realistic household environment. It features a cross-modal framework for embodied household tasks, combining high-fidelity visual environments with text-based counterparts.

\noindent \textbf{Training Setup}
We utilize Llama-3.1-8B-Instruct \cite{dubey2024llama} as the base model for verbal environments and Qwen2-VL-7B-Instruct \cite{wang2024qwen2} for vision-based tasks. Llama-3.2-Vision-11B-Instruct was excluded from our experiments due to issues with generating repetitive outputs and triggering warnings related to safety guideline violations. Detailed experimental settings and hyperparameters can be found in Appendix \ref{Experiment Settings}.

\noindent \textbf{Baselines}
To evaluate the effectiveness of our proposed method, we compare MCTS-DPO against several baselines and state-of-the-art (SOTA) agents on the ALFWorld benchmark \cite{shridhar2020alfworld}, which includes both textual and visual environments. The categorization and selection of baselines follow the methodology from EMMA \cite{yang2024embodied}. For textual environments, we evaluate three types of baselines: transformer-based models, such as BUTLER \cite{shridhar2020alfworld} and GPT-BUTLER \cite{micheli2021language}, which generate textual actions through transformer architectures; feedback-driven methods, including ReAct \cite{yao2022react}, Reflexion \cite{shinn2024reflexion}, and DEPS \cite{wang2023describe}, which leverage reasoning traces, environmental feedback, or self-explanations to refine actions; and multi-agent collaboration approaches, such as AutoGen \cite{wu2023autogen}, which enable coordination between multiple LLM agents to tackle complex tasks. For visual environments, we evaluate several baselines, including MiniGPT-4 \cite{zhu2023minigpt}, BLIP-2 \cite{li2023blip}, LLaMA-Adaptor \cite{gao2023llama}, and InstructBLIP \cite{dai2023instructblip}, which integrate visual and textual understanding through vision-language pretraining, as well as EMMA \cite{yang2024embodied}, a multi-modal agent designed specifically for embodied tasks with enhanced cross-modal reasoning capabilities.

\noindent \textbf{Evaluation Metrics}
We evaluate the performance of all methods using the following metrics: 1) Zero-Shot Success Rate: The percentage of tasks successfully completed by the agent without any fine-tuning or additional training on the evaluation tasks. 2) Average Interaction Steps: The average number of steps the agent takes to complete a task, reflecting the efficiency of the agent's decision-making process. These metrics comprehensively measure both the effectiveness and efficiency of the evaluated methods.

\subsection{Experimental Results}
\textbf{MCTS-DPO achieves SOTA in both visual and textual environments.} We evaluate MCTS-DPO against all baselines in both textual and visual environments on the ALFWorld benchmark. Results are summarized in Table \ref{tab:success rate} and Table \ref{tab:steps}, with baseline results sourced from \cite{yang2024embodied}. Our proposed method, MCTS-DPO, demonstrates clear improvements over all baselines, achieving state-of-the-art performance in both environments.

\textbf{Optimized Task Completion Rate.} MCTS-DPO outperforms all baselines in success rate, surpassing the previous textual SOTA Reflexion \cite{shinn2024reflexion} (91\%) and visual SOTA EMMA (82\%) \cite{yang2024embodied}. Notably, Reflexion and EMMA require multiple attempts to achieve their final results, whereas our method completes tasks in a single attempt, showcasing superior efficiency and robustness. These performances gains can be primarily attributed to the online nature of MCTS-DPO, which enables dynamic planning and decision-making during task execution. Online MCTS-DPO is able to handle dynamic and partially observable environments effectively. This flexibility allows the agent to generalize its strategies and maintain high success rates across diverse tasks, regardless of their complexity or dependencies.




\begin{table}[ht]
\centering
\scriptsize % 调整表格字体大小
\begin{tabular}{ccccccccc}
\hline
Type & Method & Success Rate & Pick\&Place & Clean\&Place & Heat\&Place & Cool\&Place & Look-in-Light & Pick-2\&Place \\ \hline
Text & BUTLER & 0.26 & 0.31 & 0.41 & 0.69 & 0.27 & 0.12 & 0.29 \\
Text & GPT-BUTLER & 0.69 & 0.62 & 0.81 & 0.85 & 0.78 & 0.50 & 0.47 \\
Text & ReAct & 0.54 & 0.71 & 0.65 & 0.62 & 0.44  & 0.28 & 0.35 \\ 
Text & Reflexion & 0.91 & 0.96 & 1.00 & 0.81 & 0.83 & 0.94 & \textbf{0.88} \\
Text & DEPS & 0.76 & 0.93 & 0.50 & 0.80 & \textbf{1.00} & 1.00 & 0.00 \\
Text & AutoGen & 0.77 & 0.92 & 0.74 & 0.78 & 0.86  & 0.83 & 0.41 \\
Text & IPR & 0.75 & - & - & - & - & - & - \\
\hline
Text & MCTS-DPO (Ours) & \textbf{0.92} & \textbf{1.00} & \textbf{1.00} & \textbf{0.91} & 0.80 & \textbf{1.00} & 0.67 \\
\hline

Vision & MiniGPT-4 & 0.16 & 0.04 & 0.00 & 0.19 & 0.17 & 0.67 & 0.06 \\
Vision & BLIP-2 & 0.04 & 0.00 & 0.06 & 0.04 & 0.11 & 0.06 & 0.00 \\
Vision & LLaMA-Adapter & 0.13 & 0.17 & 0.10 & 0.27 & 0.22 & 0.00 & 0.00 \\
Vision & InstructBLIP & 0.22 & 0.50 & 0.26 & 0.23 & 0.06 & 0.17 & 0.00 \\
Vision & EMMA & 0.82 & 0.71 & 0.94 & \textbf{0.85} & \textbf{0.83} & 0.88 & \textbf{0.67} \\
\hline
Vision & MCTS-DPO (Ours) & \textbf{0.87} & \textbf{0.90} & \textbf{1.00}  & 0.82  & 0.80  & \textbf{1.00} & 0.50 \\
\hline
\end{tabular}
\caption{ALFWorld Success Rate}
\label{tab:success rate}
\end{table}



\textbf{Fewer Steps, Superior Task Performance.} MCTS-DPO reduces the interaction steps to 10.22 in text and 9.9 in vision, a significant improvement compared to Reflexion’s 18 and EMMA's 19.5. 
The performance gains are primarily attributed to DPO, allowing the embodied agent to refine its commonsense understanding of the environment. This ensures that the agent focuses on the most relevant actions to achieve task objectives, avoiding unnecessary exploration. This highlights the method’s adaptability and its ability to handle the intricacies of multi-step reasoning tasks without relying on trial-and-error approaches.
This results also emphasize the model's capability to seamlessly integrate cross-modal reasoning. By leveraging its multi-modal understanding, MCTS-DPO achieves greater efficiency in environments requiring both textual and visual inputs.


\begin{table}[ht]
\centering
\scriptsize % 调整表格字体大小
\begin{tabular}{cclllllll}
\hline
Type & Method & Steps & Pick\&Place & Clean\&Place & Heat\&Place & Cool\&Place & Look-in-Light & Pick-2\&Place \\ \hline
Text & GPT-BUTLER & 18.8 & 18.4 & 18.4 & 12.7 & 15.6 & 24.4 & 26.6 \\
Text & ReAct & 20.6 & 18.1 & 18.8 & 18.2 & 23.2  & 23.7 & 25.5 \\ 
Text & Reflexion & 18.7 & 17.4 & 17.0 & 19.4 & 21.6 & 16.9 & 21.6 \\
\hline
Text & MCTS-DPO (Ours) & \textbf{10.2} & \textbf{11.5} & \textbf{9.2} & \textbf{12.3} & \textbf{8.8} & \textbf{8.7} & \textbf{11.8} \\
\hline


Vision & MiniGPT-4 & 26.9 & 29.0 & 30.0 & 26.3 & 26.7 & 17.7 & 28.9 \\
Vision & BLIP-2 & 29.5 & 30.0 & 29.3 & 29.9 & 28.2 & 29.2 & 30.0 \\
Vision & LLaMA-Adapter & 27.5 & 26.4 & 28.6 & 24.2 & 26.7 & 30.0 & 30.0 \\
Vision & InstructBLIP & 26.2 & 21.5 & 25.0 & 27.2 & 28.9 & 26.8 & 30.0 \\
Vision & EMMA & 19.5 & 19.3 & 17.5 & 19.6 & 19.9 & 19.6 & 22.4 \\
\hline
Vision & MCTS-DPO (Ours) & \textbf{9.9} & \textbf{6.8} & \textbf{10.2}  & \textbf{13.1}  & \textbf{10.9}  & \textbf{6.4} & \textbf{15.3} \\

\hline
\end{tabular}
\caption{ALFWorld Steps Counts}
\label{tab:steps}
\end{table}







\subsection{Ablation Study}
To evaluate the impact of individual components in out framwork, we conducted ablation experiments on the two key steps of MCTS-DPO: Fine-tuning with success trajectory data and DPO. The Imitation learning using expert trajectories is excluded from ablation experiments since its primary purpose is to fix output format, and it is not intended to influence performance directly. The results are presented in Table \ref{tab:ablation}

\textbf{Online Fine-tuning Enhances Accuracy.} Removing the fine-tuning step with success trajectory results in a significant drop in performanace, with success rate decreasing from 87\% to 53\%. This demonstrates the critical role of fine-tuning on success trajectory data in improving the model's ability to adapt to task-specific requirements and align its outputs with desired goals.

\textbf{DPO Improves Commonsense.} When DPO is removed, success rate remains at 87\%, same as the full framework. However, the average interaction steps increase significantly, from 9.9 to 11.8, indicating a loss in decision-making efficiency. This highlights how DPO helps refine the model’s commonsense reasoning and action prioritization, enabling the agent to make more efficient decisions during task execution.


\begin{table}[ht]
\centering
\scriptsize % 调整表格字体大小
\begin{tabular}{clllllll}
\hline
Method & Success Rate & Pick\&Place & Clean\&Place & Heat\&Place & Cool\&Place & Look-in-Light & Pick-2\&Place \\ \hline
w/o Fine-Tuning ($\mathcal{B}$) & 0.53 (8.72) & 0.6 (4.83) & 0.57 (9.5) & 0.36 (14.0) & 0.8 (9.9) & 0.56 (6.0) & 0.17 (9.0) \\
w/o DPO & 0.87 (11.8) & 0.90 (10.3) & 0.93 (9.8) & 0.91 (16.9) & 0.8 (11.4) & 1 (9.1) & 0.50 (16.7) \\
\hline
MCTS-DPO (Ours) & 0.87 (9.9) & 0.90 (6.8) & 1.00 (10.2)  & 0.82 (13.1)  & 0.80 (10.9)  & 1.00 (6.4) & 0.50 (15.3) \\
\hline
\end{tabular}
\caption{Ablation Study Result}
\label{tab:ablation}
\end{table}













==> sec/6_conclusion.tex <==
\section{Conclusion}
This paper presents MCTS-DPO, an online framework for training embodied agents that combines MCTS with DPO. Our approach address key challenges in embodied environments based on three components: (1) an efficient preference data collection method, (2) a selective state representation strategy for multi-modal reasoning, and (3) an online framework that iteratively improves model performance.

We provide theoretical analysis for our framework, proving that MCTS-based policies achieve better performance bounds. MCTS-DPO demonstrates SOTA performance in both textual and visual environments. Ablation studies highlight the roles of the framework's components: fine-tuning with success trajectories enhances task completion accuracy, while DPO significantly improves model's commonsense reasoning. These results suggest that combining MCTS-guided exploration with preference optimization creates a robust foundation for training embodied agents.

